AdaptSky: A DRL Based Resource Allocation Framework in NOMA-UAV Networks

Unmanned aerial vehicle (UAV) has recently attracted a lot of attention as a candidate to meet the 6G ubiquitous connectivity demand and boost the resiliency of terrestrial networks. Thanks to the high spectral efficiency and low latency, non-orthogonal multiple access (NOMA) is a potential access technique for future communication networks. In this paper, we propose to use the UAV as a moving base station (BS) to serve multiple users using NOMA and jointly solve for the 3D-UAV placement and resource allocation problem. Since the corresponding optimization problem is non-convex, we rely on the recent advances in artificial intelligence (AI) and propose AdaptSky, a deep reinforcement learning (DRL)-based framework, to efficiently solve it. To the best of our knowledge, AdaptSky is the first framework that optimizes NOMA power allocation jointly with 3D-UAV placement using both sub-6GHz and millimeter wave mmWave spectrum. Furthermore, for the first time in NOMA-UAV networks, AdaptSky integrates the dueling network (DN) architecture to the DRL technique to improve its learning capabilities. Our findings show that AdaptSky does not only exhibit a fast-adapting learning and outperform the state-of-the-art baseline approach in data rate and fairness, but also it generalizes very well. The AdaptSky source code is accessible to use here: https://github.com/Fouzibenfaid/AdaptSky

==> Notations.tex <==
AREA
$\mathcal{A}$ of $L \times L$ 

USERS 
$\nue=2 {N}$ number of user 
${\ue}_i$ user i  $i \in \{1,2,..\nue\}$
${\ue}_i$  and ${\ue}_{i+1}$  for $i \in \{1,3,..N \}$  best and worst channel conditions users in a given cluster 


Antenna 
$\mathcal{N}_{\uav}$ $\times$  $\mathcal{N}_{\ue}$

==> Notes_Journal.tex <==
dynamic users and adaptive clustering..

